The Fast Evolution of SN 2010bh associated with XRF 100316D

(...) Since 1998, only half a dozen spectroscopically confirmed associations have been discovered and XRF 100316D associated with the type-Ic SN 2010bh at z = 0.059 is among the latest. We began observations with GROND 12 hours after the GRB trigger and continued until 80 days after the burst. GROND provided excellent photometric data in six filter bands covering a wavelength range from approx. 350 to 1800 nm, significantly expanding the pre-existing data set for this event. Combining GROND and Swift data, the early broad-band SED is modelled with a blackbody and afterglow component attenuated by dust and gas absorption. The best-fit SED models imply moderate reddening along the line of sight through the host galaxy (A_V = 1.2 \pm 0.1 mag). The temperature and radius evolution of the thermal component are analysed and combined with earlier measurements available from the literature. This reveals a cooling envelope at an apparent initial radius of 7 \times 10^11 cm, which is compatible with a dense wind surrounding a Wolf-Rayet star. Multicolour templates of SN 1998bw are fitted to the SN to directly compare the light-curve properties. This shows that SN 2010bh is ~65% as bright as SN 1998bw. Reaching maximum brightness at ~8 days after the burst in the blue bands, SN 2010bh proves to be the most rapidly evolving GRB-SNe to date. Finally, a two-component parametrised model is fitted to the quasi-bolometric light curve, which delivers physical parameters of the explosion. This yields M_Ni = 0.21 \pm 0.03 M\bigodot and M_ej = 2.6 \pm 0.2 M\bigodot, typical of values within the GRB-SN population. The kinetic energy is 2.4 \pm 0.7 \times 10^52 erg, which is making this SN the second most energetic GRB-SN after SN 1998bw. This supernova has one of the earliest peaks ever recorded and thereafter fades more rapidly than other GRB-SNe, hypernovae, or typical type-Ic SNe. (...)

==> fBol2.tex <==
\begin{figure}
  \centering
  \includegraphics[bb=19 276 591 710,width=\linewidth,clip]{bol.eps}
  \caption{Quasi-bolometric light curve of SN 2010bh produced by using
    GROND \grizJH\ filters (black open circles) in the rest frame. For
    clarity, the uncertainties in the host-galaxy extinction are not
    included in the error bars. A single black continuous line
    represents the best-fit model (see Sect.\ \ref{ssPhy}). Early and
    late components of the model are smoothly joined at $t_0+30$~d. SE
    and other GRB-SNe quasi-bolometric light curves have been plotted
    as a comparison sample: SN 2003lw \citep[GRB
    031203;][]{Malesani04}, SN 1998bw \citep[GRB
    980425;][]{Galama98b}, SN 2006aj \citep[GRB 060218;][]{Pian06},
    the broad-lined Ic SN 2009bb \citep{Pignata11}, the type-Ic SN
    1994I \citep{Richmond96}, the type Ibc SN 2008D \citep[XRO
    080109;][]{Modjaz09,Soderberg08}, and the type-Ic SN 2002ap
    \citep{GalOfeShe02,Foley03,Yoshii03}.}
  \label{fBol}
\end{figure}

